Toward Effective Secure Code Reviews: An Empirical Study of Security-Related Coding Weaknesses

Identifying security issues early is encouraged to reduce the latent negative impacts on software systems. Code review is a widely-used method that allows developers to manually inspect modified code, catching security issues during a software development cycle. However, existing code review studies often focus on known vulnerabilities, neglecting coding weaknesses, which can introduce real-world security issues that are more visible through code review. The practices of code reviews in identifying such coding weaknesses are not yet fully investigated. To better understand this, we conducted an empirical case study in two large open-source projects, OpenSSL and PHP. Based on 135,560 code review comments, we found that reviewers raised security concerns in 35 out of 40 coding weakness categories. Surprisingly, some coding weaknesses related to past vulnerabilities, such as memory errors and resource management, were discussed less often than the vulnerabilities. Developers attempted to address raised security concerns in many cases (39%-41%), but a substantial portion was merely acknowledged (30%-36%), and some went unfixed due to disagreements about solutions (18%-20%). This highlights that coding weaknesses can slip through code review even when identified. Our findings suggest that reviewers can identify various coding weaknesses leading to security issues during code reviews. However, these results also reveal shortcomings in current code review practices, indicating the need for more effective mechanisms or support for increasing awareness of security issue management in code reviews.

==> tables/table-approach-selection-f1.tex <==
\begin{table}[ht!]
\centering
\begin{tabularx}{\linewidth}{
            >{\hsize=2\hsize}X
            >{\hsize=0.5\hsize}X
            >{\hsize=0.5\hsize}X
          }
\toprule
\textbf{Approach} & \textbf{OpenSSL} &\textbf{PHP} \\
 \midrule
 Keyword-based (KW) & 0.2807 & 0.2500 \\
 Naïve Cosine Similarity (NS) & 0.5268 & \textbf{0.4173} \\
 Soft Cosine Similarity - SO Word2Vec (SC-SO) & 0.5417 & 0.4065 \\
 % Soft Cosine Similarity - Vul Word2Vec (SC-VUL) & \textbf{0.5431} & 0.3910 \\
 \bottomrule
\end{tabularx}
\newline
\caption{F1-Score from each approach's result in each subject}
\label{table:approach_selection}
\vspace{-6mm}
\end{table}

==> tables/table-rq2-past-vulnerabilities-concern.tex <==
\begin{table}[h!]
\centering
\small
\caption{Percentage of weaknesses related to the past vulnerabilities comparing to raised security concerns in each category. The bold text indicates the categories that percentage of concerns are lower than past vulnerabilities.}
% \caption{The identified security concerns in CWE-699 categories. The bold text indicates the top 10 concerns in each project. The ${\ddag}$ symbol indicates the concerns that were frequently raised in both OpenSSL and PHP.}
\begin{tabularx}{\linewidth}{
            >{\hsize=1.2\hsize}X
            >{\hsize=0.15\hsize}X
            >{\hsize=0.15\hsize}X
            >{\hsize=0.3\hsize}X |
            >{\hsize=0.15\hsize}X 
            >{\hsize=0.15\hsize}X 
            >{\hsize=0.3\hsize}X
          }
\toprule
  \multirow{3}{*}{\textbf{Category (CWE-\#)}} & \multicolumn{3}{c|}{\textbf{OpenSSL}} & \multicolumn{2}{c}{\textbf{PHP}} \\
        & \multicolumn{2}{c}{Vuln.} & \multirow{2}{*}{\% Concern.} & \multicolumn{2}{c}{Vuln.} & \multirow{2}{*}{\% Concern.} \\
        & \# & \% & & \#  & \%  & \\
        
  \hline
    Memory Buffer Errors (1218) & \textbf{20} &  \textbf{21\%}  & \textbf{4\%}   &  \textbf{96} &  \textbf{29\%}  &  \textbf{3\%} \\
    Resource Management Errors (399) & \textbf{20} &  \textbf{21\%}  & \textbf{0\%}   & \textbf{56} &   \textbf{17\%}  &  \textbf{6\%} \\
    Information Mgmt. Errors (199) & \textbf{12} &  \textbf{13\%}  &  \textbf{3\%}   &  11 & 3\%  &  5\% \\
    Numeric Errors (189) & \textbf{8} &  \textbf{8\%}  &  \textbf{0\%}   &  \textbf{37} & \textbf{11\%}  &  \textbf{0\%} \\
    Business Logic Errors (84\%0) & \textbf{7} &  \textbf{7\%}  &  \textbf{3\%}   &  \textbf{36} & \textbf{11\%}  &  \textbf{2\%} \\
    Cryptographic Issues (310) & \textbf{7} &  \textbf{7\% } &  \textbf{4\%}   & 1 &  0.3\%   &  7\%  \\
    File Handling Issues (1219) & \textbf{7} &  \textbf{7\% } &  \textbf{1\% }  & 38 &  \textbf{12\%}  &  \textbf{3\%} \\
    Pointer Issues (465) & \textbf{6} &  \textbf{6\%}  &  \textbf{1\%}   & \textbf{29} & \textbf{ 9\%}  &  \textbf{7\%} \\
    Concurrency Issues (557) & 3 &  3\%  &  5\%   & 1 &  0.03\%   &  3\%  \\
    Data Neutralization Issues (137) & \textbf{2} & \textbf{2\%}  &  \textbf{0\%}   & 9 &  3\%  &  4\% \\
    Authentication Errors (1211) & 1 &  1\%  &  11\%   & 6 &  2\%  &  7\% \\
    Behavioral Problems (438 ) & 1 &  1\%  &  6\%   &  - & -  &  - \\
    Key Management Errors (320) & \textbf{1} &  \textbf{1\%}  &  \textbf{1\%}   &  - & -  &  -\\
    Data Processing Errors (19) & 1 &  1\%  &  3\%   &  3 & 1\%  &  2\% \\
    String Errors (133) & - &  -  &  -   &  2 & 1\%  &  3\% \\
    Type Errors (136) & - &  - &  -   &  1 & 1\%  &  3\% \\
    Other categories & - &  -  &  59\%   &  - & - &  41\% \\
    
 \bottomrule
\end{tabularx}
\newline
\label{table:rq2-past-vulnerability-concern}
\end{table}

